NeurDB: On the Design and Implementation of an AI-powered Autonomous Database

Databases are increasingly embracing AI to provide autonomous system optimization and intelligent in-database analytics, aiming to relieve end-user burdens across various industry sectors. Nonetheless, most existing approaches fail to account for the dynamic nature of databases, which renders them ineffective for real-world applications characterized by evolving data and workloads. This paper introduces NeurDB, an AI-powered autonomous database that deepens the fusion of AI and databases with adaptability to data and workload drift. NeurDB establishes a new in-database AI ecosystem that seamlessly integrates AI workflows within the database. This integration enables efficient and effective in-database AI analytics and fast-adaptive learned system components. Empirical evaluations demonstrate that NeurDB substantially outperforms existing solutions in managing AI analytics tasks, with the proposed learned components more effectively handling environmental dynamism than state-of-the-art approaches.

==> comments.tex <==
\newcommand{\comments}[2]{\begin{tcolorbox}[colback=gray!20, colframe=black, sharp corners, width=\textwidth, boxrule=0.2mm]\noindent\emph{Comment #1}: {#2}\end{tcolorbox}}
\newcommand{\response}[2]{\vspace{0mm}\noindent\textbf{Response #1}: {#2} \vspace{0.5mm}}

\newcommand{\commentsmeta}[1]{\noindent\emph{Comment}: \emph{#1}}

\newcommand{\responsemeta}[1]{\vspace{0mm}\noindent\textbf{Response}: {#1} \vspace{0.5mm}}

\newcommand{\revhighlight}[1]{\emph{\textbf{\uuline{#1}}}}
% \pagestyle{empty}
\thispagestyle{empty}


\centerline{\textbf{\Large Reviewers' Comments}}
\vspace{4mm}

% \begin{multicols}{0}

% \noindent To PC co-chairs, meta reviewer, and reviewers:




% \noindent We would like to thank the reviewers for their constructive comments and suggestions.
% We have addressed all the comments in the revised paper. 
% We highlight the major changes made on the manuscript in
% {\color{blue} blue}.



% \vspace{-3mm}
% \section*{Summary of Changes}
% \vspace{-2mm}
% \begin{itemize}[leftmargin=*,itemsep=2pt,topsep=0pt,parsep=0pt]

% \item We have revised Section~\ref{sec:application} to demonstrate how AI-powered applications in the healthcare and e-commerce domains can be potentially built with the unique functionalities of \dbname.

% \item We have addressed all the presentation issues as suggested. 
% In particular, we have revised the Abstract and Section~\ref{sec:introduction} to define the AI-powered Autonomous Data System more clearly.
% We have added the required citation in Section~\ref{subsec:related_work}.
% We have updated Figure~\ref{fig:history} and Figure~\ref{fig:overview} to enhance clarity.

% \item We have enhanced Section~\ref{subsec:auto_overview} to clarify our approach to addressing the issue that AI models can become inefficient with dynamic workloads.

% \end{itemize}
% \vspace{-2mm}



% % \section*{Response to Associate Editor}
% % % \begin{comment}
% % \commentsmeta{
% % We have now received constructive reviews for this submission. In the reviews, a common concern on the minor presentation issues has been raised. Moreover, the reviewers recommend either a minor revision or an acceptance. Based on these reviews, I recommend that this paper goes through a minor revision to fully address the reviewers’ comments.  
% % }
% % % \end{comment}


% % \responsemeta{
% % We have addressed all the minor presentation issues as suggested.
% % Furthermore, we have enhanced the paper layout and thoroughly proofread the revised paper.
% % For detailed information, please kindly refer to our responses to R1, R2, and R3 below.
% % }

% \vspace{-3mm}
\section*{Reviewer \#1}

W1. I am extremely skeptical about the need for and benefits of a learned concurrency control scheme. Even the evaluated experiment does not show particularly great scaling. Proposed model seems to have fairly high overhead to track necessary state yet benefits are not clear. I hope that authors consider expanding discussion of this component in a separate paper and evaluate it against the state of the art transaction processing systems.

W2. Regression and classification model building and evaluation has long been part of the "classic machine learning" support in all mature data management systems. It is not clear to me what is the benefit of proposing new syntax for these features instead of using existing syntax.

W3. Both industry and academia used "autonomous" to refer to operational characteristics of a database, yet the paper does not include any discussion of such concerns. It would be really interesting to discuss how newly proposed system handles both routine maintenance tasks as well as workload driven adaptation of the system configuration.

% \comments{1}{
% It is better to provide some potential applications of NeurDB, based on its unique functions.
% }


% \response{1}{
% Following your suggestion, we have improved Section~\ref{sec:application} to outline the AI-powered applications in healthcare and e-commerce domains, and envision how they can be built with the unique functionalities of \dbname.
% In addition to providing a mature infrastructure for fast data access and processing, \dbname offers in-database AI-powered analytics, which facilitates the development of complex AI applications and enhances their performance.
% }

% % In the finance sector, with \dbname, the 
% % Predict the income of all male users aged between 20 and 30.
% % Healthcare Finance
% % Multi-agent
% % RAG
% % AIGC data - data generator



% \comments{2}{
% It is better to conduct some experiments to show the performance of NeurDB.
% }

% \response{2}{
% We would like to clarify that this paper is not a full paper. It primarily focuses on positioning \dbname, our next-generation data system designed to fully embrace AI in each major system component and provide in-database AI-powered analytics.
% As mentioned in Section~\ref{sec:overview}, realizing \dbname requires significant effort in developing various techniques and evaluating \dbname necessitates a comprehensive approach that considers efficiency, security, scalability, etc. 
% To maintain a clear focus on system positioning, we chose not to include experiments in this paper.
% However, we would like to note that some key techniques used in \dbname have already been published and evaluated.
% For example, in the paper published in VLDB'24 [5], we have tested the model selection technique presented in Section~\ref{subsec:selection}.
% % ~\cite{DBLP:journals/pvldb/XingCCLOP24}
% % hard code for this citation to keep the correct citation order
% Empirical results demonstrate that our proposed technique reduces model selection time and computational expenses by up to 29.3$\times$ compared to existing model selection systems.
% Moreover, we are actively developing \dbname, and the system implementation is still in progress. 
% We shall report new experimental results as soon as they become available in the near future.
% }


% \vspace{-3mm}
\section*{Reviewer \#2}

Rename Section 2

W1. The introduction should be reworked to make it clearer earlier that the goal is to augment the functionality to allow users to make predictions rather than using AI to improve existing functionality of database internals.

W2. While I always like a good set of numbers, especially for CIDR, instead of the way that the experiments were presented, I'd rather see a more user-study type description of how using the new features helped. As is, there's not enough room to describe the experiments in the detail that such experiments need. That's okay, because I don't think the paper needs these experiments, but it would be better if the paper focused more on vision aspects.

W3. The related work section is a bit odd, since it's way shorter (and less detailed) than the discussion of related work in the intro. I'm not sure how to solve this. Perhaps my concern for W1 (about emphasizing the aspects that this work is focusing on) could be coupled with this one by moving some of that discussion into the related work section? Doing that and then moving the related work to Section 2 may address the issues nicely, but there are many possible options.

% % \begin{comment}
% \comments{1}{
% The current AI4DB actually is not fully deployed, partial due to the unstable results of AI techniques in handling the flexible input in DBMS. It is the Reliability metric in the paper. But I cannot see sufficient discussion to alleviate the issue.
% }
% % \end{comment}

% \response{1}{
% We agree that as data in the database evolves over time, static AI models can become inefficient in providing reliable results.
% To alleviate this issue, as pointed out in Section~\ref{subsec:auto_overview}, we aim to design dynamic and online AI models that can be updated and adapted to data variations to maintain accuracy, thereby facilitating the continuous optimization of system components for better performance.
% To achieve this, our core idea generally follows the FRP and employs online reinforcement learning (RL), which has been further discussed in Section~\ref{subsec:optimizer} and Section~\ref{subsec:cc}.
% We have enhanced Section~\ref{subsec:auto_overview} to state this ideation more clearly.
% % while minimizing the impact on system performance. 
% % We therefore need to design new techniques to overcome these challenges.
% % In particular, we aim to design dynamic and online AI models that facilitate continuous optimization of system components for better performance.
% }


% % \begin{comment}
% \comments{2}{
% It is better to provide the definition of Autonomous Data System at the beginning of the paper.
% }
% % \end{comment}

% \response{2}{
% Following your suggestion, we have defined the AI-powered Autonomous Data System in the Abstract and Section~\ref{sec:introduction} as a data system that provides in-database AI-powered analytics to seamlessly support AI applications, and fully embraces AI techniques in each major system component to offer self-driving capabilities.

% % We have added a period to the index terms to address this issue in the revised paper.
% }

% % \begin{comment}
% \comments{3}{
% Figure 3 gives the conceptual framework of NeurDB, while NeurDB is in the left corner in the figure. The relationships between NeurDB to other components should be more clear.
% }
% % \end{comment}

% \response{3}{
% % Thank you for pointing out the issue.
% As suggested, we have updated Figure~\ref{fig:overview} to indicate that \dbname includes Components \ding{172}\textasciitilde\ding{175}, which collaborate and interact with each other to effectively and efficiently support \ding{176} AI applications in various domains.
% % These components correspond with and interact with each other to effectively and efficiently support AI-powered applications in various domains.
% }


% \vspace{-3mm}
\section*{Reviewer \#3}

W1. In-depth discussion on the relationship between NeurDB and previous systems is needed.

W2. Both AI4DB and DB4AI are at the early stage. NeurDB (which is designed for both purposes) needs to be better motivated.

W3. NeurDB seems to be a stand-alone system or machine learning platform. More discussion on how to integrate it into database systems, e.g., PostgreSQL, is needed.

D1. NeurDB is designed to cover both AI4DB (e.g., learned database components) and DB4AI (e.g., extending SQL to answer machine learning questions) domains. In particular, Section 2.2 is about DB4AI while two AI4DB components are designed and implemented in Section 4.2. Considering that both directions are at the very early stage, the design of a system that is supposed to handle both aspects need to be better motivated. For example, is Adaptability a common issue for both of them? It seems that examples in Section 2.2 do not require “Adaptability.”

Examples about how the elements in NeurDB are assembled for both AI4DB and DB4AI tasks would be very helpful. Figure 1 is about how NeurDB is used for DB4AI tasks. It would be helpful if you can show that the same set of elements, if assembled in a different way, can support learned query optimization.

D2. NeurDB seems to be a stand-alone system or machine learning platform. If not, more discussion on how to integrate it into existing database systems, e.g., PostgreSQL, is needed. For example, if we want to deploy NeurDB on database system X, what are the assumptions about X, what kind of modifications we need to make on X, and how to connect NeurDB to X. Using PostgreSQL as an example of X to explain these questions would be very helpful.


% % \begin{comment}
% \comments{1}{
% Figure 2 AI$\times$DB looks like the English character x. Using a mathematical cross would be better.
% }

% \response{1}{
% Thank you for your careful review.
% We have revised Figure~\ref{fig:history} as suggested.
% % addressed this issue by adding a period to all the figure captions in the revised paper.
% }


% \comments{2}{
% Sec 2.3.1 Intelligent healthcare: How does that relate to DB? Though e-commerce is built on DB, how does AI$\times$DB works in e-commerce? I don't see any explicit mention of DB problems in Sec 2.3.
% }

% \response{2}{
% We have improved Section~\ref{sec:application} to clarify the relationship between modern AI applications and \dbname.
% We envision that future intelligent healthcare and e-commerce applications can be efficiently managed by \dbname, eliminating the complexity of involving multiple dedicated systems for data management, model serving, etc.
% Specifically, in the healthcare domain, the digital diagnosis system, where doctors and physicians record EMR data and other relevant patient and treatment information, can be constructed based on \dbname, which provides a mature infrastructure for fast data access and processing.
% Since all the required data is stored in \dbname, applications such as AI-powered healthcare assistants can directly perform the necessary analysis within \dbname using its in-database AI-powered analytic capabilities.
% Similarly, in the e-commerce sector, \dbname can be employed to support online purchases by maintaining tables such as the purchases data table with attributes (user, item, price).
% Based on such data tables, we can conduct various predictive tasks, such as link prediction to indicate potential purchases and fraud detection, directly within \dbname.
% }

% \comments{3}{
% In Figure 3, what's the relationship between different modules?
% }

% \response{3}{
% \dbname includes Components \ding{172}\textasciitilde\ding{175}, which collaborate and interact with each other to effectively and efficiently support \ding{176} AI applications in various domains.
% We have updated Figure~\ref{fig:overview} and the corresponding descriptions in Section~\ref{sec:framework} to state the relationship between different components more clearly.
% }

% \comments{4}{
% Do you have reference for the claim at Page 3 Line 47: Databases have the potential to efficiently manage numerous AI models using their inherent user-friendly SQL interfaces, and provide high-quality data with their transaction guarantees to enhance AI model accuracy.
% }

% \response{4}{
% To address your concern, we have added the corresponding citation for this sentence in Section~\ref{subsec:related_work}.
% }

% \twocolumn

\clearpage

==> sections/intro_bak.tex <==
\section{Introduction}

% Database management systems (DBMSs) are now the cornerstone of almost every digital platform and application across all industries.
% With DBMSs, an application developer only writes a query that specifies what data they want to access. 
% The DBMS then finds the most efficient way to store and retrieve data, and to safely interleave operations.
% DBMS can handle such data-centric tasks well until the emergence and movement of enhancing applications with artificial intelligence (AI), which is rapidly becoming mainstream with its recent advancements.
% Data, as noted by many, is the main source of knowledge that drives the intelligence of AI.


Database management systems (DBMSs) are becoming more autonomous and intelligent by embracing artificial intelligence (AI).
% With the assistance of AI, DBMSs are expected to achieve autonomous system optimization~\cite{DBLP:conf/cidr/KraskaABCKLMMN19,DBLP:conf/cidr/PavloAALLMMMPQS17,DBLP:journals/pvldb/ZhuWWWPWDLZZ24} with minimal human intervention, while supporting complex analytics~\cite{DBLP:conf/cidr/KaranasosIPSPPX20,DBLP:journals/pvldb/XingCCLOP24} for advanced data- and AI-centric applications.
AI not only empowers DBMSs to achieve autonomous system optimization with minimal human intervention~\cite{DBLP:conf/cidr/KraskaABCKLMMN19,DBLP:conf/cidr/PavloAALLMMMPQS17,DBLP:journals/pvldb/ZhuWWWPWDLZZ24,DBLP:conf/mm/WangCDGOTW15}, but also augment their functionality to support complex and advanced data analytics~\cite{DBLP:conf/cidr/KaranasosIPSPPX20,DBLP:journals/pvldb/XingCCLOP24,DBLP:conf/mm/OoiTWWCCGLTWXZZ15}, thereby catering to modern data- and AI-centric applications.
% AI empowers these systems to achieve autonomous optimization~\cite{DBLP:conf/cidr/KraskaABCKLMMN19,DBLP:conf/cidr/PavloAALLMMMPQS17,DBLP:journals/pvldb/ZhuWWWPWDLZZ24,DBLP:conf/mm/WangCDGOTW15} and support complex analytics~\cite{DBLP:conf/cidr/KaranasosIPSPPX20,DBLP:journals/pvldb/XingCCLOP24,DBLP:conf/mm/OoiTWWCCGLTWXZZ15} with minimal human intervention, thereby catering to advanced data- and AI-centric applications.

% augment the functionality to allow users to make predictions rather than using AI to improve existing functionality of database internals


% The discussion on the fusion of database systems (DB) and artificial intelligence (AI) has a long history.
The aspiration of integrating DBMSs with AI was first expressed forty years ago~\cite{DBLP:conf/aaai/Brodie88}, 
% and it has been revisited over time~\cite{DBLP:journals/sigmod/0059Z0JOT16,DBLP:conf/sigmod/CongYZ24,DBLP:conf/sigmod/ReABCJKR15}.
which has been periodically revisited with evolving technology~\cite{DBLP:journals/sigmod/0059Z0JOT16,DBLP:conf/sigmod/CongYZ24,DBLP:conf/sigmod/ReABCJKR15}.
With the advancements in both AI and DBMSs, considerable progress has been made in deepening their fusion.
Unfortunately, a huge gap remains between the potential of this integration and its current state of usability, largely due to the inherent differences in their paradigms~\cite{neurdb-scis-24}.
% Databases are dynamic in nature; the workloads they handle and the data they store continuously change over time due to user activities and interactions.
The dynamic nature of databases, characterized by constant \emph{data and workload drift}, incurs a fundamental challenge.
% For example, in an e-commerce database, it is common to experience higher loads during flash sales compared to normal periods, along with data updates resulting from customer purchases and order processing.
For example, an e-commerce database might experience %increased
a sharp increase in workloads during flash sales compared to normal periods, caused by
%frequent 
huge volumes of updates from sales transactions and processing, while the data stored in the database, such as user and product information, continuously evolves due to user activities and interactions.
% due to
%because of 
% transactional updates, and user
%activities and 
% interactions.
% In contrast, AI models typically derive intelligence from fixed and static datasets, and hence, the dynamism of databases can cause AI models to become outdated easily.
In contrast, AI models typically derive intelligence from static datasets and thus can become outdated quickly in the face of database dynamism.
For example, models for learned query optimization often acquire knowledge by training on specific system environments including data distributions and workload patterns.
% However, in case these environments drift, e.g., due to data updates, models with past knowledge can result in ineffective query optimizations because they are unaware of the new conditions.
However, when these environments drift, e.g., data distributions change due to transactional updates, models relying on past knowledge may lead to ineffective query optimizations since they are not updated to reflect new conditions.
Similarly, recommendation models trained based on historical user behaviors and product information may struggle to consistently deliver accurate product recommendations as this underlying data drifts.
% may become less accurate over time as user habits and product contexts evolve.
% Such models can become inefficient when new products are introduced or when user preferences change and these changes are not captured in the training data.



% This presents a significant challenge to ensure the AI-enhanced approaches can remain effective with dynamic workloads, and ensure AI analytics remain precise and accurate.
% Data, as noted by many, is the main source of knowledge that drives AI intelligence.
% on not only in the facets in autonomous system optimization, but also in AI  integration of AI with DBMSs, as AI models must continually adapt to changing data patterns to .

% time but lower in the daand data can be evolved over time.update and data dis
% Both AI and databases can mutually enhance each's capabilities.
% ~\cite{DBLP:journals/sigmod/0059Z0JOT16}.
% AI can assist databases to improve their performance and provide better services to support complex analytics, while databases 
% and the increasing demand for offering advanced analytics
% In this context, a series of works have been proposed. 

%Such a natural barrier 
The discrepancy in dynamicity
between AI and DBMSs 
%hinders 
poses a great challenge to
the effective adoption of AI-enhanced DBMSs.
% First, various approaches to AI-aided system optimization, 
First, traditional AI-driven system optimization,
including knob tuning~\cite{DBLP:conf/cidr/PavloAALLMMMPQS17}, 
intelligent advisors~\cite{DBLP:journals/pvldb/ZhuWWWPWDLZZ24,DBLP:journals/pvldb/0001ZSYHJLWL21}, 
and learned system components~\cite{DBLP:conf/cidr/KraskaABCKLMMN19} such as query optimizers~\cite{DBLP:conf/sigmod/MarcusNMTAK21,DBLP:journals/pvldb/ZhuCDCPWZ23}, indexes~\cite{DBLP:conf/sigmod/KraskaBCDP18}, and concurrency control~\cite{DBLP:conf/osdi/WangDWCW0021}, 
% seldom consider the dynamic workloads and data distributions.
often overlook the 
%dynamism 
dynamicity
of data and workloads.
% , which impact their effectiveness with dynamic workloads.
% Second, in-database AI analytics, another important facet of AI and DBMS integration, has gained popularity with native support for complex AI tasks such as disease progression predictions and user purchase recommendations. 
Second, another important facet of AI and DBMS integration, namely in-database AI analytics for complex tasks such as disease progression predictions and user purchase recommendations, has gained traction but faces similar adaptability issues.
% Existing works in this area typically focus on 
Existing systems generally focus on static
model inference~\cite{DBLP:journals/pvldb/SalazarDiazGR24,DBLP:conf/sigmod/ParkSBSIK22}, model serving~\cite{DBLP:conf/cidr/Vartak17}, and others~\cite{DBLP:conf/sigmod/XuQYJRGKLL0Y022},
without considering necessary model adaptations to evolving data and workload patterns.
Consequently, they require frequent manual updates and retraining to remain effective, which complicates the analytics workflow.
% However, these approaches do not account for model adaptation operations such as updates and retraining, and therefore, they need manual model adaptation to accommodate new data patterns, complicating the entire analytic workflow.
% They cannot handle model updates and retraining, making the model adaptation to new incoming data becomes rather complicated.
% for consistently precise predictions.
% Although several recent works~\cite{DBLP:journals/pacmmod/WuI24,DBLP:conf/sigmod/LiLK22,DBLP:journals/pvldb/LiWZDZ023,DBLP:journals/pacmmod/KurmanjiT23} are proposed to handle DBMS dynamism, they are effective only for specific tasks such as query optimization under read-only workloads or when data distribution changes follow certain rules.
Recent works~\cite{DBLP:journals/pacmmod/WuI24,DBLP:conf/sigmod/LiLK22,DBLP:journals/pvldb/LiWZDZ023,DBLP:journals/pacmmod/KurmanjiT23} aim to address these challenges but are typically 
%only
more
effective in controlled scenarios, such as data distribution changes following certain rules or query optimization under read-only workloads.
% Consequently, their methodologies may not generalize well to handle more practical workloads involving continuous read and write operations.
These methods
%often fail
have not been designed
to generalize across more dynamic and practical workloads involving continuous read and write operations.
% other AI-enhanced tasks and can
% Given this, designing a DBMS fully embraces AI that  remains an open problem.
% —providing AI services while being enhanced by AI—

% they are only effective on some specific tasks especially query optimization and cardinality estimization, which indicates their approaches can be infeasible for extending to other aspect of DBMS. 
% Given this, designing an efficient DBMS that truly employs AI's capability that provide AI services while being enhanced by AI can function under practical and real senarios remains an open problem.


% Systems like PostgresML~\cite{postgresml} and MindsDB~\cite{mindsdb}. 
% Several databases are proposed to integrate these learning-based techniques, such as SegaDB~\cite{DBLP:conf/cidr/KraskaABCKLMMN19} Peloton~\cite{DBLP:conf/cidr/PavloAALLMMMPQS17}, openGuess~\cite{DBLP:journals/pvldb/0001ZSYHJLWL21}.


% should combine into a single, cohesive system that can provide AI services while being enhanced by AI.
% Further, existing systems incorporate AI functionality through plugins, which can only provide AI capabilities but lack the ability to fully achieve self-optimization, making them impractical for broader use. 


% achieving the deep and real fusion of AI and DBMSs is the key to ensuring DBMSs with the integration of AI can efficiently handle dynamism.

% We envision that adapting to data and workload drifts demands the deep and real fusion of AI and DBMSs.
We envision a 
% genuine and 
deep integration of AI and DBMSs for adaptability to both data and workload drift.
% achieve the deep and real fusion of AI and DBMSs to
% Unlike current approaches that layer AI superficially atop DBMSs or selectively integrate AI into particular components, our goal is to achieve a holistic enhancement of DBMSs with AI from the ground up, enabling AI models to work closely with DBMSs to adapt to drift.
Unlike existing approaches that merely overlay AI onto DBMSs or selectively enhance certain system components, we aim for a comprehensive fusion of AI with DBMSs that enables continuous adaptation to drift.
It promises a cohesive DBMS that deeply integrates AI into each component and provides advanced in-database AI analytics.
% such an AI-powered autonomous DBMS
% However, realizing this is rather challenging.
However, achieving this level of integration presents significant challenges.
% First, fundamentally encapsulating AI into the DBMSs is complex.
% It requires a complete redesign to incorporate the entire AI workflow, including training, inference, and fine-tuning, within the database architecture.
% especially Deep Learning (DL), 
First, the integration necessitates
a fundamental redesign of the entire AI workflow, including training, inference, and fine-tuning, within the database architecture.
% Second, models for learned database components and AI analytics must rapidly adapt to drifting data workloads without sacrificing effectiveness and efficiency. 
Second, models for learned database components and AI analytics must swiftly adapt to drifting data workloads without losing effectiveness and efficiency.
% Achieving this necessitates a system foundation that supports model adaptation as well as AI models that are inherently adaptable in structure.
Therefore, developing such a system requires both a \term{system foundation that seamlessly supports model adaptation} and \term{AI models that are inherently adaptive in structure}.
% sf: check above and below paragraph - solution - ensure consistency with abstract
%shenyy: which model is ``adaptive in structure''? model is a function with a fixed structure?

% as data and workloads evolve, the model must adapt with the dynamic changes as fast as possible, yet maintain effectiveness and efficiency.
% It calls for a sophisticated system design to dynamically monitor, learn, and adjust to the changing conditions without manual intervention, and also requires AI models for both learned database components and AI analytics can fit in the adaptation framework to ensure fast adaptation.

% Due to the particular functional paradigm of different components and different AI tasks, mapping a into a particular AI algorithm is challenging
% It has statistical aggregation like functions, but does not support complex analytics and also, the existing systems hardly exploit AI to improve their perform and provide better services.
% It is about time to develop a database that achieves the deep and real fusion of AI and DB.


% \footnote[2]{\url{https://github.com/neurdb/neurdb}}
In this paper, we present \dbname, an AI-powered autonomous DBMS that provides efficient and effective in-database AI analytics to seamlessly support modern AI-powered applications, and fully embraces AI techniques in each major system component to offer self-driving capabilities.
At the core of \dbname is an in-database AI ecosystem that achieves deep integration of the AI workflow into the database.
In this ecosystem, we develop multiple in-database AI operations, such as model training, inference, and fine-tuning, along with an in-database AI engine to handle the execution of these operators.
\dbname can then directly support in-database AI analytics by calling these AI operations.
To further simplify end-users in submitting their complex AI analytics tasks to \dbname, we provide a user-friendly interface by extending SQL syntax with \texttt{PREDICT} syntax.
% We ensure these AI operators are seamlessly encapsulated within the database query executor, and therefore, \dbname to provide foundations for AI-analytics.
% , within the database architecture. 
% to ensure the accuracy and efficiency of these AI operations.
Moreover, we propose two techniques to optimize the AI ecosystem performance.
First, we devise a data streaming protocol that significantly reduces data transfer overhead, yielding better performance for AI operations.
Second, we develop an incremental update technique to minimize the fine-tuning cost, facilitating the fast adaptation of AI models.
Based on this foundation, we propose two efficient learned system components, namely a learned concurrency control algorithm and a learned query optimizer, that can adapt quickly to data and workload drift.

% , which can directly handle them.
% AI analytics can then be directly supported with such an AI ecosystem, and we enable end-users can easily submit their complex analytics tasks to \dbname by providing enhanced SQL syntax.
% We enhance the SQL syntax to provide user-friendly AI analytics service 

% to guarantee their adaptability and performance.
% AI-optimized system components.
% In particular, we present fast-adaptive deep neural ne for learned 
 % essential machine learning (ML) and deep learning (DL)
% can adapt to changing workloads dynamically and autonomously, leveraging AI to continuously monitor, learn, and optimize the system's performance.
% It is now time to develop a general-purpose AI system that can enable each end-user to benefit from the power of AI. 
% This shift towards AGI is also recognized as the continuing trend in AI development.
% Can be a strong fundamental infrastructure of realizing artificial general intelligence (AGI).


% \item We conduct extensive evaluations on the popular YCSB benchmark, and compare \dbname against OrpheusDB~\cite{orpheusdb} and Forkbase~\cite{DBLP:journals/pvldb/WangDLXZCCOR18}.
% The results show that \dbname is efficient, and it outperforms the baselines by up to 4.5$\times$.





% The remainder of the paper is structured as follows.
% The next section provides the necessary preliminaries.
% Section~\ref{sec:overview} describes the system overview of \dbname, and Section~\ref {sec:design} details the key system design, including the in-database AI ecosystem and fast-adaptive learned components.
% Section~\ref{sec:evaluation} presents the experimental results.
% Section~\ref{sec:related} discusses the related works, and Section~\ref{sec:conclusion} concludes.
